Efficient LDPC Decoding using Physical Computation

Due to 5G deployment, there is significant interest in LDPC decoding. While much research is devoted on efficient hardwiring of algorithms based on Belief Propagation (BP), it has been shown that LDPC decoding can be formulated as a combinatorial optimization problem, which could benefit from significant acceleration of physical computation mechanisms such as Ising machines. This approach has so far resulted in poor performance. This paper shows that the reason is not fundamental but suboptimal hardware and formulation. A co-designed Ising machine-based system can improve speed by 3 orders of magnitude. As a result, a physical computation approach can outperform hardwiring state-of-the-art algorithms. In this paper, we show such an augmented Ising machine that is 4.4$\times$ more energy efficient than the state of the art in the literature.

==> DAC_rebuttal.tex <==
What is the key innovation in this paper? Can you summarize it in 2-3 sentences?

1. New formulation for LDPC decode for Ising machine.

2. A detailed analysis on why existing
QUBO formulation leads to poor performance.

3. A new architecture using the proposd formulation that compares favourably with the state of the art LDPC decoders.

==> Sections/4evaluation1.tex <==
\section{Preliminary Experimental Analysis}
\label{sec:evaluations}

%The proposed LDPC decoder was simulated using MATLAB’s nonstiff, single step, 5th-order differential solver (ode45). To obtain solution quality for LDPC decoding using the QUBO formulation, we used the original BRIM model described in paper~\cite{afoakwa.hpca21} using Matlab.

Both formulations QUBO and modified QUBO were tested using Simulated annealing algorithm ~\cite{Kirkpatrick671} for solution quality. LDPC codes generated by 5G-NR standards are used as benchmarks. 

\subsection{Comparison of solution quality with QUBO Formulation }\label{sec:solution_quality}

One thousand messages were encoded using different LDPC codes to obtain the solution quality. These codes were constructed using the 5G-NR standard's base graph 1 with varying factors of expansion. The encoded messages were then modulated using BPSK modulation. The noise was added to the modulated signals based on the signal-to-noise ratio (SNR). These corrupted signals were used to test the different algorithms for solution quality. 

Figure~\ref{fig:ber} shown the solution quality of LDPC decoding using QUBO formulation and proposed formulation (modified QUBO). Both modified QUBO and QUBO were annealed using simulated annealing algorithm for 1000 iterations to obtain BER. As the simulated annealing algorithm is  probabilistic we used a different metric called Expected BER to estimate the solution quality. Each message (or instance) was annealed 100 times with random initializations. Each different anneal gives us a different solution. We find the distinct solutions in these different anneals and rank them according to their Ising energies. Considering this order static, the \textit{expected} Bit Error rate (E(BER($N_a$)))~\cite{kim2019leveraging} for each instance is calculated using the formula~\ref{eqn:expected_ber}.

\begin{equation}\label{eqn:expected_ber}
\begin{split}
E(BER(N_a)) = \sum_{q=1}^{L} \left[ (\sum_{r=q}^{L} P(r))^{N_a} -  (\sum_{r=q+1}^{L} P(r))^{N_a}\right] \\ F(q)/K    
\end{split}
\end{equation}

where K is the number of bits in the message, L is the number of unique solutions obtained by different anneals, r is the rank index of each solution, $P(r)$ is the probability of obtaining the $r_{th}$ solution, $F$ is the number of bit errors in the $q^{th}$ solution, relative to the ground truth and $N_a$ represents number of anneals. The average of 1000 different expected BER is reported as the final Bit Error rate for each SNR. As shown in the figure, modified QUBO gives us the better BER when compared to QUBO formulation.

\begin{figure}[htb]
  \centering
 \begin{minipage}[b]{.40\textwidth}
   \includegraphics[width =\textwidth]{LDPC codes/FIGS/expf_16.pdf}
  %\caption{This is first figure}
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{.5\textwidth}
  \includegraphics[width = 0.4\textwidth]{LDPC codes/FIGS/expf_2.pdf} 
  \includegraphics[width = 0.4\textwidth]{LDPC codes/FIGS/expf_4.pdf}
  %\caption{caption}
  \end{minipage} 
  \caption{Bit Error rate achieved by different algorithms at different Signal-noise ratios. Lower the better.}
\label{fig:ber}
\end{figure}

\section{Things need to be done}

\subsection{Determine accurate simulation of hardware}

The proposed hardware can be modeled using cadence but it takes lot of time to simulate. Hence we want to faithfully model the hardware using differential equation and solve it using MATLAB.

\subsection{Determine the architecture of the system}
There are two ways to determine the architecture \ding{172} to design the system to accommodate all LDPC codes determine by the standard 
\ding{173} to design the system for a particular parity check matrix
we want to explore how the system performance varies accordingly.

\subsection{Evaluate our system with state of the art LDPC decoders}

There exists plenty of literature about designing LDPC decoders. Firstly, we want to investigate if there is any advantage in decoding LDPC in our method compared to the Min-Sum algorithm. Secondly, the existing decoders are designed for different purposes using different technologies. We want to fairly compare all these decoders by adapting their design to solve a common problem and investigate how our design would compare against them.

\subsection{Noise analysis}

As our design is analog, we are prone to noise. Hence we want to investigate how our system's performance would get affected by noise. 

%\todo{To be implemented}
%\subsection{Circuit Implementation using Cadence}
%\todo{To be implemented}



==> Sections/4evaluation2.tex <==
\section{Experimental Analysis}
\label{sec:evaluations}

In this section, we discuss the experimental analysis of our design by describing benchmarks and experimental methodology and comparing our system to existing LDPC decoders in solution quality, throughput, and energy consumption. 

Existing LDPC decoders are explicitly designed to either a particular code or a standard based on a decoding algorithm. These can be implemented using GPUs, FPGAs, or as ASICs. We have surveyed the literature and chosen the state of the art ASIC decoders designed for 5G-NR standard for comparing against our design.

%The LDPC decoder designed by modifying BRIM is modeled using equation~\ref{eqn:rim_node_simplifed}. 

The proposed LDPC decoder was simulated using MATLAB’s nonstiff, single step, 5th-order differential solver (ode45). All circuits are modeled in Cadence 45nm using Generic Process Design Kit (GPDK045) to obtain power and area. To obtain solution quality for LDPC decoding using the QUBO formulation, we used the original BRIM model described in paper~\cite{afoakwa.hpca21} using Matlab.

\subsection{Comparison with existing LDPC decoders }

To compare the solution quality of different algorithms, we use a metric called Bit Error Rate (BER). It defines the probability of a bit being erroneous; mathematically, it is defined as the ratio of the number of error bits by the total number of bits. The number of error bits is equal to the Hamming distance between the decoded and original message. Lower is better.

%The LDPC decoders are designed for different standards based on other design principles using alien technology. So we decided to use $Gbits/sec/Watt$ as the final figure of merit for comparison among different LDPC decoders
%\subsection{Architectural details for 5G-NR standards}\label{sec:5g-nr}
%\subsection{Comparison with existing LDPC decoders}

\begin{comment}
\begin{table*}[htb]
\centering
\caption{comparison of hybrid LDPC decoder with existing decoders}
\label{table:comparision}
%\resizebox{\columnwidth}{!}
{
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\bf {Design\textbackslash Decoder} & \thead{~\cite{schlafer2013new}}  & \thead{~\cite{lin202133}} & \thead{~\cite{cheng2014fully}}   & \thead {~\cite{lee2022multi}}  & \thead{~\cite{thi2021low}} & \thead{this work}\\  
\hline\hline

CMOS Technology  &   65nm LVT  & 28nm & 90nm   & 65nm  & 65nm & 45nm\\ 
\hline
Standard        &  IEEE802.11ad   & 5G-NR   & -    &5G-NR & 5G-NR & 5G-NR \\ 
\hline
Decoding Algorithm & Min-Sum & \thead{ Normalized\\Min-Sum}   &  \thead{ Normalized\\Min-Sum}  & \thead{ offset\\Min-Sum} & \thead{Combined \\ Min-Sum} & \thead{hybrid \\ Ising model}  \\
\hline
Block size         &  672  &  \thead{all cases of 5G}  & 2048 & \thead{all cases of 5G} & 3808 & \thead{all cases of 5G} \\
\hline
\thead{Decoding Latency \\(iterations or annealing time) }  &  10 & 5 &  9 & 3 &10 & 0.22 $\mu sec$\\
\hline
Max Throughput (GBs/sec) & 160.8 & 6.7  & 45.09  & 21.78 &3.04 & 118.6 \\
\hline
Max Power (mW)    & 5360 & 232 & 1110 & 413 & 259 & 1566 \\
\hline
Area ($mm^2$) &   12.09  & 1.97 & 9.6 & 5.74 & 1.49 & 33\\
\hline
Energy (pJ/bit)  & 36.1 & 145  & 20.33  & 94.89 & 85.2& 13.14\\

%\hline
%Gbits/Sec/$mm^2$  & 13.30 & 3.4  & 4.7  & 3.82 & 2.04& -\\
%\hline

\hline
\end{tabular}
}
\end{table*} 


\subsection{Comparison with existing LDPC decoders}

\begin{table*}[htb]
\centering
\caption{comparison of hybrid LDPC decoder with existing decoders}
\label{table:comparision}
%\resizebox{\columnwidth}{!}
{
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{|c|c|c|c|c|c|} 
\hline
\bf {Design\textbackslash Decoder} & \thead{~\cite{schlafer2013new}}  & \thead{~\cite{lin202133}}   & \thead {~\cite{lee2022multi}}  & \thead{~\cite{thi2021low}} & \thead{this work}\\  
\hline\hline

CMOS Technology  &   65nm LVT  & 28nm   & 65nm  & 65nm & 45nm\\ 
\hline
Standard        &  IEEE802.11ad   & 5G-NR & 5G-NR & 5G-NR & 5G-NR \\ 
\hline
Decoding Algorithm & Min-Sum & \thead{ Normalized\\Min-Sum}   &  \thead{ offset\\Min-Sum} & \thead{Combined \\ Min-Sum} & \thead{hybrid \\ Ising model}  \\
\hline
Block size         &  672  &  \thead{all cases of 5G}  & \thead{all cases of 5G} & 3808 & 1088 \\
\hline
\thead{Decoding Latency per iteration\\ (nsec)} &  4  & 787 & 1530  & 125.33  & 220  \\
\hline
\thead{Max Throughput per iteration \\(GBs/sec)} & 160.8 & 33.2  & 17.06 & 30.38 & 4 \\
\hline
Max Power (mW)    & 5360 & 232  & 413 & 259 & 6.59 \\
\hline
Area ($mm^2$) &   12.09  & 1.97  & 5.74 & 1.49 & - \\
\hline
Energy (pJ/bit) per iteration  & 36.1 & 29  & 24.2 & 8.52 & 1.33\\
\hline
\thead{BER @ SNR 3 \\ exp\_factor = 16 \\ bit width =8bits }  &  5.69E-02 & \red{3.67E-02}  & 3.67E-02 & \red{3.67E-02} & 1.61E-02\\
\hline
\end{tabular}
}
\end{table*}
\end{comment}

\todo{block size must be the same, increase either area or latency to compensate for the block size, equation}


\note{equation of energy per bit: (power*latency)/number of bits }
\note{Time : SA = 1340ms; OMS = 1.4ms; ~\cite{thi2021low}=752ns; BRIM style ldpc\_decoder = 220ns}

\note{Solving G001: number of nodes: 800 
SA : number of instructions 2388227818
Number of spin flips: 220759
Total time per flip: (total number of instr per flip*time per cycle)/IPC

Assumming IPC: 2
total number of instr per flip = 10818
clk speed =  3 GHz  0.33ns
Total time per flip: $(10818*0.33*10^(-9))/2 = 2e-06$

BRIM: total time 2.2e-06
Number of spin flips: 105660
Total time per flip in BRIM : 2e-11

so total speedup = 2e-06/2e-11 = $10^5$

}

\note{minsum on cpu could solve in 1.4ms, ~\cite{thi2021low} solve in 752ns, approx 3 orders of speed up compared to cpu, compared to SA BRIM\_ldpc\_decoder is $6.5*10^6$ X faster approximated by scaling}

\note{ Explaining the speedup: ~\cite{thi2021low} has 56X19 functional units which is 3 orders more functional units compared to cpu.
}

\note{100 Messages SNR:3; exp\_f:2 each message was annealed 20 times

      1) annealing time 1.5 $\mu s$, number of anneals 1, BER: 5.11E-03;
      
      2 a) annealing time 300ns, number of anneals 5, total time 1.5 $\mu s$ BER: 7.05E-03;
      
      2 b) start from end result 

      2 c) start from hard decision point. 
      
      annealing time 150ns, number of anneals 9 and 1 anneal to get to the energy point at 150ns in total annealing time of approx 1.5 $\mu s$ BER: 8.85E-03

      annealing time 270ns, number of anneals 5  1 anneal to get the energy point at 30ns in total annealing time of 300ns total time 1.380 $\mu s$ BER:7.29E-03
}


\begin{table}[htb]
\centering
\caption{comparison of hybrid LDPC decoder with existing decoders, all parameters are adjusted to implement highest lifting size}
%\resizebox{\columnwidth}{!}
\label{table:comparision}
\resizebox{\columnwidth}{!}{
\setlength{\tabcolsep}{4pt}

\label{table:comparision}
{
\begin{tabular}{|c|c|c|c|c|} 
\hline
\bf {Design\textbackslash Decoder}  & \thead{~\cite{lin202133}}   & \thead {~\cite{lee2022multi}}  & \thead{~\cite{thi2021low}} & \thead{this work}\\  
\hline\hline

CMOS Technology    & 28nm   & 65nm  & 65nm & 45nm\\ 
\hline
Standard          & 5G-NR & 5G-NR & 5G-NR & 5G-NR \\ 
\hline
Decoding Algorithm & \thead{ Normalized\\Min-Sum}   &  \thead{ offset\\Min-Sum} & \thead{Combined \\ Min-Sum} & \thead{hybrid \\ Ising model}  \\
\hline
Block size         &  26112 & 26112 & \red{26112} & \red{26112} \\
\hline
\thead{Decoding Latency per iteration\\ (nsec)}  & 787 & 1530  & \red{860}  & \red{220}  \\
\hline
\thead{Max Throughput per iteration \\(GBs/sec)}  & 33.2  & 17.06 & \red{30.36} & \red{118.6} \\
\hline
Max Power (mW)     & 232  & 413 & 259 & \red{158.24} \\
\hline
Area ($mm^2$)  & 1.97  & 5.74 & 1.49 & \red{5.44} \\
\hline
Energy (pJ/bit) per iteration   & 29  & 24.2 & \red{8.52} & \red{1.33}\\
\hline
%BER SNR 1.5 & 4.3797e-07 & 7.4420e-05 & - &-\\
%\hline
%quantization   & 5  & 8  & 4 & -\\
%\hline
%metric  & -  & -  & - & -\\
%\hline

\end{tabular}
}
}
\end{table}

Table ~\ref{table:comparision} shows a detailed comparison of our work with existing ASIC LDPC decoders. These ASIC LDPC decoders are designed for 5g-NR standards with different technologies. They are designed by hard-wiring different variations of the Min-Sum algorithm. ~\cite{lin202133}, ~\cite{thi2021low} can implement all the codes defined by the standard where as ~\cite{thi2021low} is designed for a specific expansion factor 56. For fair comparison we converted all the numbers reported to represent an implementation of an LDPC code constructed using base graph 1 with an expansion factor of 384 and with a code rate of 1/3. 

In base graph 1 with an expansion factor of 384, there are $121344$ non zero entries. So to construct our decoder we need $121344*2$ xnor gates and $26112$ capacitors. The gates and capacitors are connected to from $17664$ parity equation and $26112$ nodes. The annealing time 220ns is estimate by obtaining same bit error rate as of offset Min-sum algorithm at different SNRs for one iteration. For same annealing time we estimated the power consumption to be 158.24mw. According to the table we can see that there is 6.4X reduction in energy consumption per bit.


\begin{comment}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{LDPC codes/FIGS/perfomance_ldpc.pdf}
    \caption{Performance vs Power Consumption of various LDPC decoders implemented in literature}
    \label{fig:ldpc_results}
\end{figure}

Figure~\ref{fig:ldpc_results} shows the graph of throughput vs power consumption of ASIC LDPC decoders. The graph is obtained from the following survey papers ~\cite{kingston2021certain,maunder2016survey}. \blue{Even in this graph, all the LDPC decoders are designed with different technology and for different standards. The graph shows that power consumption grows exponentially with the growth in throughput. In our design, parity units are responsible for most power consumption. They grow linear to the expansion factor. Hence, using our design, we could achieve linear growth in power consumption with throughput.}
\end{comment}


\subsection{Comparison of solution quality with QUBO Formulation }\label{sec:solution_quality}

One thousand messages were encoded using different LDPC codes to obtain the solution quality. These codes were constructed using the 5G-NR standard's base graph 1 with varying factors of expansion. The encoded messages were then modulated using BPSK modulation. The noise was added to the modulated signals based on the signal-to-noise ratio (SNR). These corrupted signals were used to test the different algorithms for solution quality. 

Figure~\ref{fig:ber} shown the solution quality of LDPC decoding using QUBO formulation and proposed algorithm (modified QUBO). Both modified QUBO and QUBO were annealed for 0.22$\mu$s to obtain BER. As both QUBO and modified QUBO are probabilistic we used a different metric called Expected BER to estimate the solution quality. Each message (or instance) was annealed 100 times with random initializations. Each different anneal gives us a different solution. We find the distinct solutions in these different anneals and rank them according to their Ising energies. Considering this order static, the \textit{expected} Bit Error rate (E(BER($N_a$)))~\cite{kim2019leveraging} for each instance is calculated using the formula~\ref{eqn:expected_ber}.

\begin{equation}\label{eqn:expected_ber}
\begin{split}
E(BER(N_a)) = \sum_{k=1}^{L} \left[ (\sum_{r=k}^{L} P_I(r))^{N_a} -  (\sum_{r=k+1}^{L} P_I(r))^{N_a}\right] \\ F_I(k)/N     
\end{split}
\end{equation}

where N is the number of bits in the message, L is the number of unique solutions obtained by different anneals, r is the rank index of each solution, $P_I(r)$ is the probability of obtaining the $r_{th}$ solution, and $F_I$ is the number of bit errors in the $k^{th}$ solution, relative to the ground truth. The average of 1000 different expected BER is reported as the final Bit Error rate for each SNR. As shown in the figure, modified QUBO gives us the best BER when compared to QUBO formulation.

\begin{figure}[htb]
  \centering
 \begin{minipage}[b]{.40\textwidth}
   \includegraphics[width =\textwidth]{LDPC codes/FIGS/expf_16.pdf}
  %\caption{This is first figure}
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{.5\textwidth}
  \includegraphics[width = 0.4\textwidth]{LDPC codes/FIGS/expf_2.pdf} 
  \includegraphics[width = 0.4\textwidth]{LDPC codes/FIGS/expf_4.pdf}
  %\caption{caption}
  \end{minipage} 
  \caption{Bit Error rate achieved by different algorithms at different Signal-noise ratios. Lower the better.}
\label{fig:ber}
\end{figure}

\section{Things need to be done}

Need to evaluate if BRIM can obtain same Bit Error rate as of Offset Min-Sum algorithm at higher iterations. 

Need to determine the actual architecture of the system.

Perform Noise analysis


\todo{To be implemented}

%\subsection{Circuit Implementation using Cadence}

%\todo{To be implemented}



==> Sections/7notes.tex <==
\todo{Find out performance/energy of ``baseline Ising machine" so that we can discuss this improvement in abstract.}
\note{According to the following paper "https://arxiv.org/abs/2007.11069" a 2048 qbit dwave machine can implement a 420bit problem, which can achieve 0.021 gbits/sec  throughput. Whereas state of the art machines achieve 33.2 gbits/sec and we achive 81.6 gbits/sec}

\note{
expansion factor 4, binary;  number of spins: 689 , couplers: 15616; unary, number of spins: 1029 , couplers 25148; actual spins (our model) 272, couplers 1264\\
expansion factor 64, binary; number of spins:11009 ,
Couplers:290688; unary number of spins: 16449, couplers: 443200; acutal spins (our model) 4352.0, couplers 20224.
}

\note{ SNR = power of signal / power of noise; (No units, generally expressed in dB)

$N_0/2$ is the power spectral density of noise;

2W be the bandwidth;

P be the power of signal;

power of noise = $N_0/2*2W$ = $N_0*w$

so SNR = $P/N_0*W$

If 2W is the bandwidth of the signal, Time required to transmit a symbol without interference (T) = $1/2W$ (According to Nyquist rate)

So energy per symbol $(E_s)$ = P*T =  $P/2W$

The energy of noise = variance of noise ($\sigma^2$) = $N_0/2$; (This is derived)

so $E_s/\sigma^2$ = $P/N_0*W$ = SNR;

For BPSK Modulation

Energy per symbol = mean of square of symbol = $((-1)^2 + (1)^2)/2 = 1$

Hence SNR = $1/\sigma^2$

In an uncoded transmission number of information bits = number of symbols, Hence rate (R) = 1, but in a coded transmission R < 1, so to transmit same amount of information we need to use more energy in coded transmission compared to uncoded transmission. 

To have fair comparison between coded and uncoded we use a metric called $E_b/N_0$ instead of SNR,

$E_b$ = Energy per bit = $E_s/R$ = $(E_s*n)/k$

SNR = $E_s/sigma^2$ = $2*R*E_b/N_0$

$E_b/N_0 = 1/(2*R*\sigma^2)$

From the above formula we can calculate sigma for the noise based on $E_b/N_0$ value.

}
\note{equation of energy per bit: (power*latency)/number of bits }
\note{Time : SA = 1340ms; OMS = 1.4ms; ~\cite{thi2021low}=752ns; BRIM style ldpc\_decoder = 220ns}

\note{Solving G001: number of nodes: 800 
SA : number of instructions 2388227818
Number of spin flips: 220759
Total time per flip: (total number of instr per flip*time per cycle)/IPC

Assumming IPC: 2
total number of instr per flip = 10818
clk speed =  3 GHz  0.33ns
Total time per flip: $(10818*0.33*10^{(-9)})/2 = 2e-06$

BRIM: total time 2.2e-06
Number of spin flips: 105660
Total time per flip in BRIM : 2e-11

so total speedup = 2e-06/2e-11 = $10^5$

}

\note{minsum on cpu could solve in 1.4ms, ~\cite{thi2021low} solve in 752ns, approx 3 orders of speed up compared to cpu, compared to SA BRIM\_ldpc\_decoder is $6.5*10^6$ X faster approximated by scaling}

\note{ Explaining the speedup: ~\cite{thi2021low} has 56X19 functional units which is 3 orders more functional units compared to cpu.
}

\note{100 Messages SNR:3; exp\_f:2 each message was annealed 20 times

      1) annealing time 1.5 $\mu s$, number of anneals 1, BER: 5.11E-03;
      
      2 a) annealing time 300ns, number of anneals 5, total time 1.5 $\mu s$ BER: 7.05E-03;
      
      2 b) start from end result 

      2 c) start from hard decision point. 
      
      annealing time 150ns, number of anneals 9 and 1 anneal to get to the energy point at 150ns in total annealing time of approx 1.5 $\mu s$ BER: 8.85E-03

      annealing time 270ns, number of anneals 5  1 anneal to get the energy point at 30ns in total annealing time of 300ns total time 1.380 $\mu s$ BER:7.29E-03
}


==> Sections/DAC_rebutal.tex <==
What is the key innovation in this paper? Can you summarize it in 2-3 sentences?

The key innovations in this paper are:

1) Observation: Mapping Ising machines onto Ising machines by converting into QUBO formulation would result in bad performance.

Innovations:
New formulation of LDPC decoding to map onto Ising machines by designing a higher order ising machines
 
The design of LDPC decoder based on new formulation 

Comparison with state of the art LDPC decoders 



==> backup/background.tex <==
\section{Background and Related Work}
\label{sec:background}
In this section, we discuss LDPC codes, the decoding algorithm of LDPC codes, the Ising model, conversion of decoding problem into a QUBO, and existing Ising machines.
\section{Background}
\subsection{Low Density Parity Check Code}
Low Density Parity Check codes are a class of linear block codes. The parity bits (redundant information) are obtained using bitwise XOR operation on a selected number of message bits. These codes are specified by a generator matrix $G_{k \times n}$ and a parity check matrix $H_{m \times n}$~\footnote{can be obtained from another by using the following relation $H\xor G^\top =0$}. The name Low Density comes from the sparse structure of the parity check matrix. The Generator matrix is used for encoding a message ($M$) into a code word (C) using the following equation $C = G^\top \xor M$. $m$ is a number of parity bits, $n$ is the total number of bits in the encoded code word, and $k$ is the number of bits in a message ($k=n-m$). The ratio of the length of the message (k) to the size of the code word (n) is called Rate (r) = $k/n$. At the receiver side the decoded message is obtained from both received message (R) and the parity check matrix.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.38\textwidth]{FIGS/tanner_graph.pdf}
    \caption{Tanner graph constructed using parity check matrix H shown in figure.}
    \label{fig:tg}
\end{figure} 

LDPC codes can be represented graphically using Tanner graphs. These graphs are bipartite, meaning that the graph nodes are separated into two distinctive sets, and edges only connect nodes of two different types. The two types of nodes in a Tanner graph are variable and check nodes. Figure \ref{fig:tg} is an example of a Tanner graph that is constructed using parity check matrix H shown above. It consists of m check nodes (the number of parity bits) and n variable nodes (the number of bits in an encoded message). Check node $P_i$ is connected to variable node $c_j$ if the element $h_{ij}$ of H is a 1. These graphical structures are handy for analysis and decoding purposes.

There are many LDPC codes like regular, irregular, systematic, and nonsystematic. In regular code, the degree of rows and columns of parity check matrix are equal, i.e., the number of ones in rows and columns are identical. In a systematic code, an encoded message is constructed with message bits followed by parity bits. The main advantage of systematic code is that the message can be directly obtained from the decoded code word. Most commonly used LDPC codes are irregular systematic codes. These codes can also be constructed using a base graph as a template; hence they are called protographic.

\subsection{Binary Phase shift Keying}
To efficiently transmit messages over communication channels, modulation schemes are employed. In this paper, we consider binary phase-shift keying (BPSK). This technique utilizes a single-frequency carrier signal and encodes digital data onto the signal by applying a phase shift. For a 0 in the data, no phase shift is applied; for a 1, the phase of the carrier signal is shifted by $180$ degrees. The data can then be recovered by the receiver by simply checking for the presence of this shift during each clock cycle by comparing it to a reference signal. If the carrier during that period has a phase shift present, the transmitted bit is decoded as 1; if not, the transmitted bit is decoded as 0.

%\todo{I could explain more here and go into tradeoffs of using BPSK if you want, but I felt this keeps it simple and is enough to understand the uses of BPSK in the paper}

% I'm not sure if this mathematical explanation is really necessary to get the point across, and introducing more equations can serve to complicate the paper if they're not really required
 
Mathematically, encoding a message using BPSK modulation can be represented as follows. If $M$ is the message used for transmission, $S$ is the modulated signal, then $S = 1-2 \times M$. The received signal $R$ can be defined as $R= S+ n$, where $n$ is the noise added to the signal by the channel. 

\subsection{Decoding LDPC codes using Belief Propagation}

LDPC codes are decoded using \textit{belief propagation} algorithm. The code word $\tilde{C}$ is decoded from the received message by calculating each bit's belief, or log-likelihood ratio (LLR), of being zero. The LLR of each bit of codeword has two components: intrinsic ($LLR_I$) and extrinsic ($LLR_E$). An intrinsic component of a bit $i$ (${LLR_I}_i$) is calculated using the corresponding bit ($R_i$) in the received message. The extrinsic component is calculated using the rest of the bits of the received message.

The decoding process of LDPC code uses tanner graph representation. First, the tanner graph variable nodes are initialized using the intrinsic LLRs, and these values are broadcasted to the neighboring check nodes. An extrinsic LLR is calculated at each check node based on the received LLRs from other adjacent variable nodes for each neighboring variable node. Once the calculation is done, the extrinsic LLRs are again broadcasted back to each corresponding neighboring variable node. After receiving the extrinsic LLRs from the check nodes, LLRs are recalculated for each connected check node using both received extrinsic LLRs from other check nodes and the intrinsic LLR of that variable node. Once the calculation is done, it is broadcasted again to check nodes. This passing process is carried out until the maximum iteration count is attained or until the decoded code word can satisfy the parity check conditions. This decoding methodology is also popularly known as a message-passing algorithm.

Let us assume the received message is $R$ of length $n$ been transmitted over a channel with additive white Gaussian noise and the signal is modulated using BPSK modulation scheme. It is encoded using LDPC code (k, n). Let us also assume the decode code word be $\tilde{C}$. Let the set of variable nodes that are connected to check node $c$ be denoted as $N(c)$, and the set of check nodes that are connected to variable node $v$ be denoted as M(v). Also $N(c)\backslash v$ and $M(v)\backslash c$ denote the set N(c) and M(v) excluding bit node v and check node c. The conventional iterative decoding process is based on the following steps:

%\note{A couple of ambiguities. $\tilde{c}$ is the decoded word, which means M+N bits long? But $c$ is a "node"? meaning it's not a word or related to word $\tilde{c}$, using deliberately the same letter implied some connection -- that one is a variation of the other.}

Step 1:

Each variable node v, is initialized using the intrinsic log-likelihood ratio  calculated by using following formula, 

\begin{equation}
    LLR_{I_{v_i}} = \log \frac{P(v_i=0/R_i)}{P(v_i=1/R_i)} = \frac{2R_i}{\sigma^2} 
\end{equation}

%\note{$0/r_i$ is still 0. Do you mean conditional probability given $r_i$}

where $\sigma$ represents the estimated variance of the Gaussian noise of the channel and $P(v_i=0/R_i)$ conditional probability of $v_i$ being zero, given $R_i$.
%\note{Do you mean estimated/assumed variance}

Step 2:

Once the LLR values are calculated at variable nodes, they are passed to the neighboring check nodes. Let $LLR_{c,v}$ be the LLR received by the check node $c$ from variable node $v$.

At the check node $c$ for each neighboring variable node $v$, an extrinsic LLR ($LLR_{v,c}$) is calculated  using equation~\ref{eq::llrc2v} and passed to that corresponding node.

\begin{equation}
%\begin{split}
    \label{eq::llrc2v}
    LLR_{v,c} = 2 \times \arctanh\{   \\ \prod_{v_{i} \in N(c)\backslash v}  \frac{1+e^{-|LLR_{c,v_{i}}|}}{1-e^{-|LLR{c,v_{i}}|}}\}
%    \end{split}
\end{equation}

Step 3:

After receiving the messages from the check nodes, the extrinsic messages to the neighboring check nodes are computed using equation ~\ref{eq::llrv2c} and passed to corresponding check nodes.

\begin{equation}
    \label{eq::llrv2c}
    LLR_{c,v} = \sum_{c_{i} \in M(v)\backslash c} LLR_{v,c{_i}} + LLR_{I_{v}}
\end{equation}

The value of each bit of code word is decided at the variable node by calculating the final LLR by summing all LLRs received from the check nodes along with the intrinsic LLR. If the final LLR value is greater than zero, then the value of the bit is decided as zero; otherwise, 1. Step2 and Step3 are repeated until a maximum number of iterations are reached or if the decoded code word satisfies the constraint $H \xor c =\hat{0}$.

($LLR_{v,c}$) calculated using equation~\ref{eq::llrc2v} is approximately equal to the minimum absolute value of the LLRs received from variable nodes. The sign of $LLR_{v,c}$ is equal to the product of the sign of $LLR_{c,v}$ with the product of all received LLRs. 

Based on this approximation, a variation of the Belief propagation called the Min-Sum algorithm was developed. The LLRs that need to be propagated to the neighboring variable node are calculated by replacing all the received LLRs with the minimum value, and the minimum value is replaced with the second minimum value. The product of the signs of received LLRs decides whether to flip the signs or not.

\subsection{Ising Model}\label{sec:ising_mode}
The Ising model is used to describe the Hamiltonian \ie the total energy, of a system of coupled
spins. The spins have one degree of freedom and take one of two values ($+1$,
$-1$). The energy of the system is a function of pair-wise coupling of the
spins ($J_{ij}$) and the interaction ($h_i$)
of some external field ($\mu$) with each
spin. The resulting Hamiltonian (Energy function)~\footnote{In this context we use Hamiltonian and energy function interchangeably.} is as follows:

\begin{equation}
\label{eqn:Ising_w_field}
% H = -\sum_{(i<j)} J_{ij}\sigma_i\sigma_j - \mu \sum_i h_i\sigma_i
E = -\sum_{\mathclap{(i<j)}} J_{ij}\sigma_i\sigma_j - \mu \sum_{\mathclap{i}} h_i\sigma_i
\end{equation}


A physical system with such a Hamiltonian naturally tends towards low-energy
states. It is as if nature tries to solve an optimization problem with
Eq.~\ref{eqn:Ising_w_field} as the objective function, which is not a trivial
task. Indeed, the cardinality of the state space grows exponentially with the
number of spins, and the optimization problem is NP-complete: it is easily
convertible to and from a generalized max-cut problem, which is part of the
original list of NP-complete problems~\cite{Karp1972}.

Thus if a physical system of spins somehow offers programmable coupling
parameters ($J_{ij}$ and $\mu h_i$ in Eq.~\ref{eqn:Ising_w_field}), they can
be used as a special purpose computer to solve\footnote{Throughout
the paper, by ``solving" an optimization problem we mean the
searching for a good solution rather than necessarily finding the global optimum, 
equivalent to reaching the ground state.} optimization problems that
can expressed in the form of an Ising formula (Eq.~\ref{eqn:Ising_w_field}). In fact, all
problems in the Karp NP-complete set have their Ising formula
derived~\cite{lucas2014ising}. Also, if a problem already has a QUBO (quadratic
unconstrained binary optimization) formulation, mapping to Ising formula is as
easy as substituting bits for spins: $\sigma_i = 2b_i-1$.

Because of the broad class of problems that can map to the Ising formula,
building nature-based computing systems that solve these problems has
attracted significant attention~\cite{kim2010quantum,berloff2017realizing,
barends2016digitized,yamaoka201520k,bunyk2014architectural,king2018observation,
bohm2019poor,hamerly2019towards,pierangeli2019large}.
Loosely speaking, an Ising machine's design goes through four
steps:
\begin{enumerate}

\item Identify the physical variable to represent a spin (be it a 
qubit~\cite{PhysRevB.82.024511}, the phase of an optical pulse~\cite{inagaki2016coherent}, 
or the polarity of a capacitor's voltage~\cite{afoakwa.hpca21}).

\item Identify the mechanism of coupling and how to program the coefficients.

\item Demonstrate the problem solving capability showing both the theory of its
operation (reveal the ``invisible hand" of nature) and satisfactory results
of practice.

\item Demonstrate superior machine metrics (solution time, energy consumption,
and construction costs).

\end{enumerate} It is important to note that different approaches may
offer different fundamental tradeoffs and goes through varying gestation
speeds. Thus it could be premature to evaluate a general approach based on
observed instances of prototypes. Nevertheless, we provide a broad-brushed
characterization, which can help researchers get a 
basic sense of the landscape -- as long as the caveats are properly understood.

\subsection{Decoding of LDPC codes to QUBO} \label{sec:QUBO_formulation}

The decoding of LDPC codes can be modeled as a combinatorial optimization problem with the following objectives. The decoded codeword $\tilde{C}$ should be closer to the received message and should satisfy the parity check matrix. If we use the BPSK modulation scheme, the objective function can be represented by the following equation~\ref{eq::obj}.

\begin{comment}
\begin{equation}
\label{eq::obj}
\begin{split}
    F = \sum_{i=0}^{n-1}(R_i - (1-2\tilde{C_i}))^2 \\
   with\ constraint\ that\  H \xor \tilde{C} = \hat{0}
\end{split}
\end{equation}
\end{comment}

\begin{equation}
\label{eq::obj}
\begin{split}
    F = \sum_{i=0}^{n-1}(R_i - (1-2\tilde{C_i}))^2 +  (H \xor \tilde{C})
\end{split}
\end{equation}
The higher order function XOR operation in equation~\ref{eq::obj} poses constraints in this problem. Mapping a combinatorial optimization problem with higher order terms on an Ising Machines needs to be converted into a  Quadratic Unconstrained binary optimization (QUBO). There are many ways of this conversion, but here we discuss one of the conversions, which uses minimum auxiliary spins~\cite{tawada2020new}. The constraint in the objective function of LDPC decoding is that modulo2 (or XOR operation) of matrix-vector multiplication of parity check matrix $H$ and $\tilde{C}$ must result in a vector of zeros. It means that the dot product of each row of the parity check matrix with $\tilde{c}$ must result in an even number. It can be represented as $H_j \cdot \tilde{C} = 2L_j$, where j is a row of parity check matrix(H), and $L_j$ is some arbitrary integer.

This condition can be represented using the following objective function

\begin{equation}
    F_s = \sum_{j=1}^{m}(\sum_{i=1}^{n} H_{j,i}\tilde{C}_i - 2L_j)^2
\end{equation}

Consider encoding an arbitrary integer $L_j$ with auxiliary variables
$y_{j,k}$ where $y_{j,k} \in \{0,1\}$. If the number of 1’s in $H_j$ is $|H_j|$, the range of $L_j$ is $0 \leq l \leq \lfloor \frac{|H_j|}{2} \rfloor $. $L_j$ can be encoded using either the unary encoding or the binary encoding as follows 

\begin{itemize}
    \item Unary encoding \\
             $L_j = \sum_{k=0}^{\lfloor \frac{|H_j|}{2} \rfloor} y_{j,k}$
    \item Binary encoding \\
             $L_j = \sum_{k=0}^{\lfloor \log_2 (\frac{|H_j|}{2})\rfloor} 2^k y_{j,k}$
\end{itemize}

so the objective function can be written as 

\begin{equation}
\label{eq::obj_ising}
\begin{split}
    F = \sum_{i=0}^{n-1}(R_i - (1-2\tilde{C_i}))^2 + \alpha F_s
\end{split}
\end{equation}

~\cite{tawada2020new} suggested to chose $\alpha > \sum_{i=1}^{n} 4|R_i|$. In our observation using this equation resulted in poor results, hence we enumerated alpha values and chose the one which gave us good result.

F can be written in the following format: $F = x^\top Qx +c$ where $x$ represents the variables of $\tilde{C}$ and auxiliary variables $y_{j,k}$. The matrix $Q$ is mapped on to Ising machines to find $X$ that results in optimal solution of $F$.  

As we can see, the conversion of LDPC decoding into a QUBO problem requires extra spins, which increases the size of the problem.

\subsection{Ising Machines}

We divide existing Ising Machines into three categories based on the technology used for their design: Quantum, Optical, and Electronic annealers. 

The latest Quantum Ising annealer manufactured by D-wave can support up to 2000 qubits~\cite{D-Wave}. The qubits are coupled to form a chimera graph. As a result of local coupling, the D-wave machine can only map up to 64 nodes all to all connected graph~\cite{hamerly2019experimental, hamerly2018scaling}. These annealers are also susceptible to noise, necessitating cryogenic operating condition that consumes much power (25KW for D-Wave 2000q)~\cite{dwave_stats}.

The Most popular optical-based Ising machine is the Coherent Ising Machine (CIM)~\cite{inagaki2016cim, cim_yamamoto, McMahon614, 16bit_cim, ncomm_bohm2019}. It uses an optical parametric oscillator to generate and manipulate the signal to represent one spin. Unlike D-Wave, CIM nodes are all-to-all coupled. The machine has two components: an optical cavity built using kilometers of fibers, and an auxiliary computer to implement coupling between nodes. Every pulse's amplitude and phase in the optical cavity are detected, and its interaction with all other pulses is calculated using an auxiliary computer (FPGA). This computation is then used to modulate new pulses that are injected back into the optical cavity. Strictly speaking, the current implementation is a nature-simulation hybrid Ising machine. Thus, beyond the challenge of constructing the cavity, CIM  also requires a significant supporting structure that involves fast conversions between optical and electrical signals. 


 The operating principle of CIM can be viewed as a Kuramoto model~\cite{Takeda_2017},  so in theory, we can achieve a similar goal using other oscillators. This led to the design of an electronic Oscillator-based Ising Machines. These systems use LC tanks for spins and (programmable) resistors as coupling units. However, inductors are often a source of practical challenges for on-chip integration. They are area intensive and have undesirable parasitics with reduced quality and increased phase noise, which poses practical challenges in maintaining frequency uniformity and phase synchronicity between thousands of on-chip oscillators. 


Another electronic design with resistive coupling is the Bistable Resistively-coupled Ising Machine (BRIM)~\cite{afoakwa.hpca21}, in which the Ising spin is implemented as capacitor voltage controlled by a feedback circuit, making it bistable. Since it uses voltage (as opposed to phase) to represent spin, it enables a straightforward interface to implement additional architectural support for computational tasks. In BRIM, the polarity of the voltage across a capacitor represents the spin of the node and the coupling strength is inversely proportional to the resistance of the coupling resistors, i.e., $R_{ij}=\frac{R}{\abs{J_{ij}}}$, where $R$ is a scaling coefficient and the negative coupling is achieved by cross coupling the capacitors in neighboring nodes.

\begin{comment}
\subsection{Existing LDPC decoders}
\todo{need to discuss about existing hardware LDPC decoders and existing Ising machines }

Most of the LDPC decoders in literature are designed by a hard-wiring a specific algorithm for a particular parity check matrix based on a chosen standard. ~\cite{?} discuss the design of LDPC decoder for 5g standard implementing offset Min-Sum Layered algorithm. The following design only supports the LDPC decoder for 5g base graph1 with an expansion factor of 384. ~\cite{?} discuss the design of the same 5g standard LDPC decoder implementing the same offset Min-sum algorithm but with support for all graphs possible in the standard. ~\cite{?} discuss pipelining the layered Min-sum algorithm for IEEE 802.e. standard to achieve high throughput.

Ising Machines have also been used for implementing decoders for LDPC codes. ~\cite{?} discuss how to convert LDPC codes into QUBO format and implement LDPC codes on D-wave. This implementation's main drawback is that it cannot fit an LDPC code of standards. This system's bit error rate (BER) is not as good as the Min-Sum algorithm's.
\end{comment}

==> backup/conclusion.tex <==
\section{Conclusions}\label{sec:conclusion}

In this paper we explained about

\begin{itemize}
    \item  LDPC codes are important ECC codes for its ability to reach the Shannon limit
    \item they have been standardized for many different applications
    \item The decoding of LDPC codes is a combinatorial optimization problem
    \item Ising machines have shown to solve COPs very effectively
    \item major problem: to map cop with constraints on ising machines needs to be converted into a QUBO which requiers some extra spins
    \item this makes the state space for search increase exponentially
    \item with changes to the hardware of BRIM we can directly map decoding LDPC without conversion
    \item this leads to design of LDPC decoder with \blue{118.6 Gbits/sec} through, \blue{158.24mW} power consumption.
    \item this design helps in reduction of energy consumption per bit by an order of magnitude compared to other state of art LDPC decoders
    
\end{itemize}

==> backup/evaluation.tex <==
\section{Experimental Analysis}
\label{sec:evaluations}

In this section, we discuss the experimental analysis of our design by describing benchmarks and experimental methodology and comparing our system to existing LDPC decoders in solution quality, throughput, and energy consumption. %\blue{We will also provide a circuit simulation using cadence as a proof of concept}. 
Existing LDPC decoders are explicitly designed to either a particular code or a standard based on a decoding algorithm. These can be implemented using GPUs, FPGAs, or as ASICs. We have surveyed the literature and chosen the state of the art ASIC decoders designed for different standards for comparing against our design.

The LDPC decoder designed by modifying BRIM is modeled using equation~\ref{eqn:rim_node_simplifed}. We performed simulations using MATLAB’s nonstiff, single step, 5th-order differential solver (ode45). All circuits are modeled in Cadence 45nm using Generic Process Design Kit (GPDK045) to obtain power and area. To obtain solution quality for LDPC decoding using the QUBO formulation, we used the original BRIM model described in paper~\cite{afoakwa.hpca21} using Matlab. 

\subsection{Benchmarks and Metrics}

They are many standards defining LDPC codes for different applications. Most recently, the LDPC code has been standardized for wireless enhanced-mobile broad-band (eMBB) communication in 5G new radio (NR) by the 3-generation partnership project (3GPP). We use the LDPC codes defined by this standard as our benchmarks to compare the solution quality of different algorithms.

\begin{figure}[htp]
    \centerline{\includegraphics[width=0.47\textwidth]{LDPC codes/FIGS/circular_shift.pdf}}
    \caption{Structure of 5G-NR standard base graph 1. Each blue dot represents a nonzero element which will be replaced by a circular identity matrix based on the expansion factor as shown.}
    \label{fig:5g-nr}
\end{figure}

\subsubsection{5G-NR standard} \label{sec:5g_nr_standard}
 The 5G standard describes two base-graph (BG) matrices: BG1 and BG2, which are used to construct a parity check matrix. Figure~\ref{fig:5g-nr} shows the structure of BG1. The blue dots in the figure~\ref{fig:5g-nr} show nonzero elements of the matrix. It has 46 rows and 68 columns, and the BG2 matrix has 42 rows and 52 columns. Rows in the base graphs describe parity check equations. By default, BG1 generates an LDPC code with a rate equal to $1/3$, and BG2 generates an LDPC code with a rate equal to $1/5$. Based on the required rate, we chose the base graph. 

Once the base graph is chosen, each zero entry is replaced with a $Z \times Z$ all-zero matrix. Each nonzero entry is replaced with a $Z \times Z $ circular shifted identity matrix. $Z$ is called an expansion factor. The amount of circular shift depends on the value of the nonzero element. The values of the nonzero elements range from 0 to z. If the value is 0, replace the element with the $Z \times Z$ identity matrix; otherwise, circularly shift the identity matrix based on the value. In figure ~\ref{fig:5g-nr} an example with an expansion factor of 4 and the circular shift amount of 2 is shown. The 5G-NR standard allows different discrete expansion factors ranging from 2 to 384. For any further details please refer to the following paper~\cite{bae2019overview}.

\subsubsection{Metrics}

To compare the solution quality of different algorithms, we use a metric called Bit Error Rate (BER). It defines the probability of a bit being erroneous; mathematically, it is defined as the ratio of the number of error bits by the total number of bits. The number of error bits is equal to the Hamming distance between the decoded and original message. Lower is better.

%The LDPC decoders are designed for different standards based on other design principles using alien technology. So we decided to use $Gbits/sec/Watt$ as the final figure of merit for comparison among different LDPC decoders

%\subsection{Architectural details for 5G-NR standards}\label{sec:5g-nr}




%\subsection{Comparison with existing LDPC decoders}

\begin{comment}
\begin{table*}[htb]
\centering
\caption{comparison of hybrid LDPC decoder with existing decoders}
\label{table:comparision}
%\resizebox{\columnwidth}{!}
{
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\bf {Design\textbackslash Decoder} & \thead{~\cite{schlafer2013new}}  & \thead{~\cite{lin202133}} & \thead{~\cite{cheng2014fully}}   & \thead {~\cite{lee2022multi}}  & \thead{~\cite{thi2021low}} & \thead{this work}\\  
\hline\hline

CMOS Technology  &   65nm LVT  & 28nm & 90nm   & 65nm  & 65nm & 45nm\\ 
\hline
Standard        &  IEEE802.11ad   & 5G-NR   & -    &5G-NR & 5G-NR & 5G-NR \\ 
\hline
Decoding Algorithm & Min-Sum & \thead{ Normalized\\Min-Sum}   &  \thead{ Normalized\\Min-Sum}  & \thead{ offset\\Min-Sum} & \thead{Combined \\ Min-Sum} & \thead{hybrid \\ Ising model}  \\
\hline
Block size         &  672  &  \thead{all cases of 5G}  & 2048 & \thead{all cases of 5G} & 3808 & \thead{all cases of 5G} \\
\hline
\thead{Decoding Latency \\(iterations or annealing time) }  &  10 & 5 &  9 & 3 &10 & 0.22 $\mu sec$\\
\hline
Max Throughput (GBs/sec) & 160.8 & 6.7  & 45.09  & 21.78 &3.04 & 118.6 \\
\hline
Max Power (mW)    & 5360 & 232 & 1110 & 413 & 259 & 1566 \\
\hline
Area ($mm^2$) &   12.09  & 1.97 & 9.6 & 5.74 & 1.49 & 33\\
\hline
Energy (pJ/bit)  & 36.1 & 145  & 20.33  & 94.89 & 85.2& 13.14\\

%\hline
%Gbits/Sec/$mm^2$  & 13.30 & 3.4  & 4.7  & 3.82 & 2.04& -\\
%\hline

\hline
\end{tabular}
}
\end{table*} 
\end{comment}

\subsection{Comparison with existing LDPC decoders}

\begin{table*}[htb]
\centering
\caption{comparison of hybrid LDPC decoder with existing decoders}
\label{table:comparision}
%\resizebox{\columnwidth}{!}
{
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{|c|c|c|c|c|c|} 
\hline
\bf {Design\textbackslash Decoder} & \thead{~\cite{schlafer2013new}}  & \thead{~\cite{lin202133}}   & \thead {~\cite{lee2022multi}}  & \thead{~\cite{thi2021low}} & \thead{this work}\\  
\hline\hline

CMOS Technology  &   65nm LVT  & 28nm   & 65nm  & 65nm & 45nm\\ 
\hline
Standard        &  IEEE802.11ad   & 5G-NR & 5G-NR & 5G-NR & 5G-NR \\ 
\hline
Decoding Algorithm & Min-Sum & \thead{ Normalized\\Min-Sum}   &  \thead{ offset\\Min-Sum} & \thead{Combined \\ Min-Sum} & \thead{hybrid \\ Ising model}  \\
\hline
Block size         &  672  &  \thead{all cases of 5G}  & \thead{all cases of 5G} & 3808 & \thead{all cases of 5G} \\
\hline
\thead{Decoding Latency \\(iterations or annealing time) }  &  10 & 5 & 3 &10 & 0.22 $\mu sec$\\
\hline
Max Throughput (GBs/sec) & 160.8 & 6.7   & 21.78 &3.04 & 118.6 \\
\hline
Max Power (mW)    & 5360 & 232  & 413 & 259 & 158.24 \\
\hline
Area ($mm^2$) &   12.09  & 1.97  & 5.74 & 1.49 & 33\\
\hline
Energy (pJ/bit)  & 36.1 & 145  & 94.89 & 85.2& 1.34\\

%\hline
%Gbits/Sec/$mm^2$  & 13.30 & 3.4  & 4.7  & 3.82 & 2.04& -\\
%\hline

\hline
\end{tabular}
}
\end{table*}


\subsubsection {Comparison with ASIC LDPC decoders}
Table ~\ref{table:comparision} shows a detailed comparison of our work with existing ASIC LDPC decoders. All the parameters reported in the table are directly obtained from their papers. 

These ASIC LDPC decoders use different standards and different technologies. They are designed by hard-wiring different variations of the Min-Sum algorithm. 

We designed our BRIM-based LDPC decoder to implement all the codes defined by the 5G-NR standards. The maximum expansion factor allowed by 5G standards is 384, and the maximum number of columns and rows are 68 and 46, respectively. If we construct a code using these factors, it results in a parity check matrix of size $17664 \times 26112$. Suppose we choose a naive design to accommodate this parity check matrix. In that case, we require a system with $26112$ nodes and $17664 \times 26112 = 461242368$ parity units. As described in section~\ref{sec:5g_nr_standard}, the nonzero elements are replaced by a circular shift identity matrix. So even if we consider all $46 \times 68$ matrix to be nonzeros, maximum, we require $46 \times 68\times 384=1024512$ parity units. So to reduce the space and energy, we designed our system with $26112$ rows but $46$ columns. Each row would represent a node, and each column would represent $384$ parity equations. To represent these parity equations, we need $384\times 2$ different wires in each column. If we layout our chip with 45nm technology using four metal layers, 27 $\mu$m wide~\footnote{According to the following paper~\cite{sicard2011introducing} in 45nm technology in metal layers, 1 to 4, the wire width is 60nm, and the space between wires is 80nm}.
If we consider the parity units to be $1\mu$m in length, then the total area of the chip would be 33$mm^2$ approximately. The total annealing time to decode a code word is $0.22 \mu s$, which results in a throughput of 118.6 Gbits/sec. We calculated the maximum power consumed by this system to be 158.24 mW~\footnote{There are 316 nonzero elements in base graph 1. So only $316X384 = 121344$ parity units will be active for a parity check matrix constructed using an expansion factor of 384.}. Hence from this design, we can at least achieve an order of magnitude reduction in energy consumption per bit when compared to other state of the art designs.


\begin{comment}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{LDPC codes/FIGS/perfomance_ldpc.pdf}
    \caption{Performance vs Power Consumption of various LDPC decoders implemented in literature}
    \label{fig:ldpc_results}
\end{figure}

Figure~\ref{fig:ldpc_results} shows the graph of throughput vs power consumption of ASIC LDPC decoders. The graph is obtained from the following survey papers ~\cite{kingston2021certain,maunder2016survey}. \blue{Even in this graph, all the LDPC decoders are designed with different technology and for different standards. The graph shows that power consumption grows exponentially with the growth in throughput. In our design, parity units are responsible for most power consumption. They grow linear to the expansion factor. Hence, using our design, we could achieve linear growth in power consumption with throughput.}
\end{comment}
%\subsubsection{Comparison with existing Ising machines}

%As discussed in the following section~\ref{?} after conversion, the problem size of 5G-NR LDPC code with an expansion factor of 384 increases to \blue{48769} spins. 

%\todo{need to write}

\subsection{Comparison of solution quality of different algorithms }\label{sec:solution_quality}

One thousand messages were encoded using different LDPC codes to obtain the solution quality. These codes were constructed using the 5G-NR standard's base graph 1 with varying factors of expansion. The encoded messages were then modulated using BPSK modulation. The noise was added to the modulated signals based on the signal-to-noise ratio (SNR). These corrupted signals were used to test the different algorithms for solution quality. 

In Figure~\ref{fig:ber} labels 1 to 10 represent the maximum number of iterations used for decoding in the Min-Sum algorithm. QUBO represents the decoding of LDPC codes using QUBO formulation. Modified QUBO represents LDPC decoding using the proposed design. Both modified QUBO and QUBO were annealed for 0.22$\mu$s to obtain BER. The Min-sum algorithm is deterministic, whereas QUBO and modified QUBO are probabilistic. So, we used a different metric called Expected BER to estimate the solution quality. Each message (or instance) was annealed 100 times with random initializations. Each different anneal gives us a different solution. We find the distinct solutions in these different anneals and rank them according to their Ising energies. Considering this order static, the \textit{expected} Bit Error rate (E(BER($N_a$)))~\cite{kim2019leveraging} for each instance is calculated using the formula~\ref{eqn:expected_ber}.

%Figure ~\ref{fig:ber} shows the Bit Error Rate (BER) of different algorithms at different SNR values. The titles of each graph show the expansion factor used for creating the LDPC codes.

\begin{equation}\label{eqn:expected_ber}
\begin{split}
E(BER(N_a)) = \sum_{k=1}^{L} \left[ (\sum_{r=k}^{L} P_I(r))^{N_a} -  (\sum_{r=k+1}^{L} P_I(r))^{N_a}\right] \\ F_I(k)/N     
\end{split}
\end{equation}

 

where N is the number of bits in the message, L is the number of unique solutions obtained by different anneals, r is the rank index of each solution, $P_I(r)$ is the probability of obtaining the $r_{th}$ solution, and $F_I$ is the number of bit errors in the $k^{th}$ solution, relative to the ground truth. The average of 1000 different expected BER is reported as the final Bit Error rate for each SNR. As shown in the figure, modified QUBO gives us the best BER when compared to all the other algorithms.

\begin{figure}[htb]
  \centering
 \begin{minipage}[b]{.40\textwidth}
  \includegraphics[width=\textwidth]{LDPC codes/FIGS/2_.pdf}
  %\caption{This is first figure}
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{.5\textwidth}
  \includegraphics[width = 0.32\textwidth]{LDPC codes/FIGS/4_.pdf}
  \includegraphics[width = 0.32\textwidth]{LDPC codes/FIGS/8_.pdf} 
  \includegraphics[width = 0.32\textwidth]{LDPC codes/FIGS/16_.pdf}
  %\caption{caption}
  \end{minipage} 
  \caption{Bit Error rate achieved by different algorithms at different Signal-noise ratios. Lower the better.}
\label{fig:ber}
\end{figure}

\subsection{Impact of circuit element's noise on solution quality}

\todo{To be implemented}

%\subsection{Circuit Implementation using Cadence}

%\todo{To be implemented}

==> backup/intro.tex <==
\section{Introduction}

Error-correcting codes (ECCs) are used to control data errors over unreliable or noisy communication channels. The central idea is that the sender encodes the message with redundant information in the form of an ECC. The redundancy allows the receiver to detect a limited number of errors that may occur anywhere in the message and often correct them without the need for retransmission. These codes are used in communication systems for reliable transmission and computer memories for reliable storage. There have been many ECCs introduced in the literature, such as Hamming codes ~\cite{hamming1950error}, convolutional codes~\cite{viterbi1971convolutional}, polar codes~\cite{arikan2008performance}, turbo codes~\cite{berrou1993near}, etc. However, among them, low density parity check (LDPC) codes have become more popular due to their ability to achieve the Shannon limit~\cite{mackay1999good}. 

These codes were introduced by Robert Gagllaer in 1962~\cite{gallager1962low} and are used in various applications and standards. Recently they have been introduced in the 5G-NR standard along with Polar codes~\cite{bae2019overview}. Decoding LDPC codes is a combinatorial optimization problem with constraints. Many algorithms like the sum of products and belief propagation have been developed to solve this problem. These algorithms calculate the belief of a bit being one or zero. The Min-Sum algorithm, an approximation to belief propagation, is most popular among digital ASIC designers.

In a related but different track of work, researchers are trying to solve a combinatorial optimization problem by mapping to physical processes such that the resulting state represents an answer to the problem. Quantum computers marketed by D-Wave Systems are prominent examples. Unlike circuit model quantum computers~\cite{google_quantum,pednault2019leveraging}, D-Wave machines perform quantum annealing~\cite{bunyk_2014_tas}. The idea is to map a combinatorial optimization problem to a system of qubits such that the system's energy maps to the metric of minimization. Then, when the system is controlled to settle down to a low-energy state, the qubits can be read out, which correspond to a solution of the mapped problem.

Indeed, several alternative designs have emerged recently, showing good quality solutions for non-trivial sizes in milli- or micro-second latencies~\cite{inagaki2016cim, wang2019oim, carmes_comm2020}. These systems all share the property that a problem can be mapped to the machine's setup. Then the machine's state evolves according to the physics of the system. This evolution has the effect of optimizing a formula called the Ising model (more on that later). 
Hence they are called Ising Machines. Reading out the state of such a system at the end of the evolution thus has the effect of obtaining a solution (usually a very good one) to the problem mapped. 

%Quadratic Unconstrained binary optimization (QUBO) problem. 
%Bistable Resistively-coupled Ising Machine (BRIM) is a CMOS-compatible Ising machine that is shown to outperform many existing Ising machines~\cite{afoakwa.hpca21}, which we use as a baseline system.

LDPC decoding can be formulated as an optimization problem for a standard Ising machine. However, the problem itself is a form of constrained optimization. A standard formulation approach causes the problem size to 
be doubled. 
As the state space of in a combinatorial optimization increases 
exponentially with regard to the problem size, such increase in problem
size comes with devastating impact on any solvers.
In this paper, we address this problem by modifying the hardware of 
a state-of-the-art electronic Ising machine so that it more efficiently
solve LDPC decodes without drawback from the standard formulation approach.
The proposed modification helps to achieve an LDPC decoder with a 
throughput of \blue{118 Gbits/sec} and a power consumption of \blue{158.24mW}, 
representing at least an order of magnitude reduction in energy compared to state-of-the-art decoders for 5G standards.

==> backup/proposed.tex <==
\section {Architecture}
\label{sec:arch}


%In this section, we discuss about the algorithm change to QUBO formulation of decoding of LDPC codes and it's formulation.

\subsection{Intuition}



\subsubsection{Modifications to QUBO formulation}\label{secc:m_qubo}The state space for an Ising model scales with $2^n$ where $n$ is the number of nodes, also referred to as the problem size. The number of  auxiliary spins required for QUBO formulation discussed in section ~\ref{sec:QUBO_formulation} is almost equal to number of spins in the problem\footnote{ For binary representation, unary representation requires more.}. This causes a considerable problem for solution quality (which will be shown in a following section, ~\ref{sec:solution_quality}), as well as wasting hardware. So we have come with a new methodology of mapping LDPC decoding problems without any conversion. The XOR operation can be converted into a multiplication operation by replacing 0 with 1 and 1 with -1. It can be seen in the following truth table: Table ~\ref{tabel:truth_table}. 

\begin{table}[h]\centering
\caption{Conversion of XOR operation into multiplication  }
\label{tabel:truth_table}
\begin{tabular}{|c|c|c|c|c|c|} 
\hline
$A$ &  $B$ &  $A \xor B$ & $\sigma_A$ & $\sigma_B$ & $\sigma_A.\sigma_B$ \\ 
\hline\hline
 0 &  0  & 0 & 1 & 1 & 1\\  
\hline
0  &  1 & 1 & 1 & -1 & -1\\   
\hline
1    & 0 & 1 & -1& 1& -1\\ 
\hline
1    & 1 & 0  & -1 & -1 & 1\\ 
\hline
\end{tabular}
\end{table}

Hence the equation~\ref{eq::obj} can be written as follows:

\begin{equation}
\label{eq::mul_obj}
\begin{split}
    f = \sum_{i=0}^{n-1}(R_i - \tilde{C_i})^2  + \sum_{j=0}^{m-1}(1-(\Pi_{i=0}^{n-1} H_{i,j} \tilde{C_i}))/2
\end{split}
\end{equation}

by removing constants equation~\ref{eq::mul_obj} can be written as:

\begin{equation}
\label{eq::LDPC_ising}
\begin{split}
    f = \sum_{i=0}^{n-1}-2r_i\tilde{C_i}  - \sum_{i=0}^{n-1}\sum_{j=0}^{m-1} H_{i,j} \tilde{C_i} P_{j\backslash i} \\
    where\ P_{j\backslash i}\ =\ \Pi_{k=0 \backslash i }^{n-1} H_{k,j} \tilde{C_k}
\end{split}
\end{equation}


We can see that equation~\ref{eq::LDPC_ising} bears a significant resemblance to the Ising model described in section~\ref{sec:ising_mode} where $P_{j\backslash i}$ is a higher order term. So we modified BRIM to implement these higher order terms so that we could map LDPC codes without conversion.


\subsubsection{Hardware representation}


Consider 1 (0) to be high and -1 (1) to be low in the above truth table~\ref{tabel:truth_table}. The output ($\sigma_A.\sigma_B$) represents an XNOR logic. %~\footnote{ The output is high when both inputs are the same, and low when inputs are different}. 
Hence $P_{j\backslash i}$ can be calculated by XNORing the state of node $V_i$ with parity equation $P_j$. 
The parity equation can be evaluated by XNORing the states of nodes involved. In equation~\ref{eq::LDPC_ising}, for simplicity, if we consider that the system energy only depends upon satisfying the parity equations. If a parity equation is satisfied, the current states of nodes that make it up should not be changed. Otherwise, they should be flipped so that the equation will be satisfied. This behavior can be easily mimicked using the circuit shown in Figure~\ref{fig:circuit_digaram}.

\begin{figure}[htp]
    \centerline{\includegraphics[width=0.40\textwidth]{LDPC codes/FIGS/circuit_diagram.pdf}}
    \caption{Logical implementation of proposed LDPC decoder }
    \label{fig:circuit_digaram}
\end{figure}

We can consider that Figure~\ref{fig:circuit_digaram} shows the circuit implementation of equation~\ref{eq::LDPC_ising} with a parity check matrix that has only one parity equation. The voltage on capacitors represents the states of nodes. The parity equation $P$ is implemented by XNORing all the nodes involved \ie, $V_1$ to $V_4$. $P_{\backslash i}$ at each node is calculated by XNORing the state of node $V_i$ with parity equation $P_j$.

Suppose we consider $P$ being satisfied when it is high. In the figure, when $P$ is high, the output of XNOR gates, connected to the capacitor of nodes representing $P_{\backslash i}$, is the same as that of the node's states. So when a parity equation P is satisfied, the states of nodes $V_1$ to $V_4$ are not changed. When the parity equation ($P$) is low,  $P_{\backslash i}$ contradicts the node's states. So the output of XNOR gates will flip the states of nodes. Hence this circuit can find a code word that satisfies a parity equation. 

 To achieve the code word closer to the received message, we can apply a bias voltage at each node representing the received message. The sign of the received message determines whether to charge or discharge the node. The amount of charging or discharging depends on the value of the message.

By modifying the coupling units and nodes to implement the above circuit, we can directly map the LDPC decoding problem to BRIM without converting it into a QUBO.


\subsection{Architecture of hybrid LDPC decoder}
\label{ssec:arch}

We now discuss the architectural changes made to BRIM to implement an LDPC decoder. The system is illustrated in Fig.~\ref{fig:BRIM_arch} and consists of: 
\ding{172} bistable nodes (V1 to V4) and their digital interface (DFF 1-4); 
\ding{173} parity units connecting the nodes ($PU_{ij}$); \ding{174} 
programming units to configure parity units (including: memory, multiplexers,
digital-to-analog converters, and the column control systems); and \ding{175} annealing control. The rows (i) represent the variable nodes, and the columns (j) represent check nodes in a Tanner graph. Row $i$ is used for calculating $\sum_j P_{j\backslash i}$ of a node $i$ by summing the output currents from parity units of that row. Column $j$  is used to evaluate the parity equation "$P_j$." We discuss each unit in turn as follows:

\begin{figure}[htp]
    \centerline{\includegraphics[width=0.45\textwidth]{LDPC codes/FIGS/ldpc_new_arch.pdf}}
    \caption{Block diagram of BRIM based LDPC decoder's system components. Nodes are $N_i$ and parity units $PU_{i,j}$. The multi-colored interconnecting links are wires}
    \label{fig:BRIM_arch}
\end{figure}

\subsubsection{\bf Nodes}

We slightly modified bistable nodes $v_i$ of BRIM to implement biasing. In Fig.~\ref{fig:node_and_iv} we show a more detailed illustration of one node. A ZIV diode is used as the feedback circuit to stabilize the voltages at the desired levels (\eg $\pm V_{dd}$). The figure shows the IV curve of the ZIV diode. When capacitor voltages are in between $-V_{dd}$ and $V_{dd}$, the diode acts as an active element charging its voltage closer to $\pm V_{dd}$. Conversely, for voltages outside the range, the ZIV diode acts essentially as a linear resistor to discharge the capacitor. 

Each node is supplied with two pairs of switches to set the capacitor voltage to a known spin state. It is helpful for specific initialization or to change the system state as described in the  "Annealing Control "(Sec.~\ref{ssec:anneal_control}). Finally, the spin of the node can be read 
out by a digital latch (\eg a D flip-flop) connected to the ZIV diode's 
$V+$ terminal. It converts the spin to a bit (1 or 0). The pins labeled $V+$, and $V-$ are used to connect to the parity units' inputs and outputs. The bias determined by the received message is applied as a voltage through resistors (B+, B-) as shown in figure~\ref{fig:node_and_iv}. The value of resistance depends upon the value and sign of the received message.

%If the sign of the message is positive, switch B+ is turned on, and B- is turned off, and vice versa. These switches are programmed using the programming pin.

\begin{figure}[htp]\centering
\includegraphics[width=0.28\textwidth]{LDPC codes/FIGS/variable_node.pdf}
\includegraphics[width=0.20\textwidth]{ziv_curve.pdf}
\caption{Simplified schematic of one BRIM node (left) and ZIV diode's IV 
characteristic (right). \label{fig:node_and_iv}}
\end{figure}

\subsubsection{\bf Parity Unit}

The parity unit ($PU_{ij}$) represents the coupling unit in BRIM. Here, it is used for coupling node $V_i$ to parity equation $P_j$ and vice versa. It has the following functionalities \ding{172} to determine value $P_{j \backslash i}$ and pass it to node $V_i$ ,\ding{173} to evaluate the parity equation $p_j$ if node $V_i$ is connected to parity equation $P_j$, otherwise just pass the previous value of $P_j$ value to other nodes in same column.

 As shown in Fig ~\ref{fig:PU} an XNOR gate (X1) with inputs $V_i+$ and $P_j^{in}$ are used to determine function \ding{172}. The output of the gate X1 is connected to $V_i-$ via a programmable coupling resistor ($T_1$) which acts as a switch. The programmable coupling resistor is implemented using a transistor whose charge on gate capacitance determines if the switch is on or off. According to parity equation $P_j$, if node $V_i$ is involved, then the switch $T_1$ would be turned on; otherwise, off. \ding{173} function is implemented using another XNOR gate (X2). As shown in Fig ~\ref{fig:PU} the inputs of XNOR (X2) gate are $P_j^{out}$ and $V_i+$.  $P_j^{out}$ represents the value of the parity equation ($P_j$) determined by the previous nodes in the column. If node $V_i$ is involved in the equation, then the node's current state should be XNORed with $P_j^{out}$ to determine the final value. If it is not involved in the equation, we should pass the value on to other nodes. To implement this, we used two switches $T_2$ and $T_3$ operating conversely. If node $V_i$ is involved then $T_2$ is turned on and $T_3$ is off; otherwise $T_3$ is turned on and $T_2$ is left off. These coupling resistors are programmed using a row selector and a column selector, which will be discussed in the next section. After determining the final value of $P_j$, it is passed as input to the parity units to calculate $P_j\backslash i$. The nodes c1, c2, and c3 in Figure~\ref{fig:BRIM_arch} represent the connection of wires between the $P_j^{out}$ and $P_j^{in}$. In this way, we have changed the architecture, nodes, and coupling unit structure of BRIM to directly map the LDPC decoding problem to the system. The rest of the unit's functionality is the same as BRIM, but we discuss it here also.
 
\begin{figure}[htp]
    \centerline{\includegraphics[width=0.5\textwidth]{LDPC codes/FIGS/parity_unit_ldpc.pdf}}
    \caption{Schematic of parity unit. Color schemes are matched to system-level block diagram in Fig ~\ref{fig:BRIM_arch} }
    \label{fig:PU}
\end{figure}

\subsubsection{\bf Programming units}
Both the initial nodal values and the coupling resistances in parity units are programmable.
Programming of a resistor is achieved through a transistor with adjustable 
gate voltage.
% The details of the circuit design are discussed in Appendix~\ref{ ssec:circuit}. 
To the right of the parity unit array in 
Fig.~\ref{fig:BRIM_arch} is the programming array. This array consists of 
digital memory for storing the weights which drive an array of digital-to-analog 
converters (DACs).

A small amount of such DACs are sufficient to program all the parity units in a time-interleaved fashion per column. In such configuration, 
we need corresponding column selectors and pull-down logic as shown below 
the coupling units in Fig.~\ref{fig:BRIM_arch}.

\subsubsection{\bf Annealing control}\label{ssec:anneal_control}

As our system is primarily an optimizer, it can get stuck in local minima. To avoid this, two commonly used mechanisms for annealers were adopted and incorporated to allow the system to escape local optima. First, the coupling strength is globally increased over time. In this way, at the very beginning, the machine is only weakly coupled, rendering the energy landscape relatively flat. It helps the system explore the landscape in a coarse granularity. We choose an exponential annealing schedule because (a) it is a common practice, and (b) it can be conveniently achieved by discharging an appropriately-sized capacitor as the global annealing scheduler. The voltage from this capacitor is then used to control the variable gain buffer in each node to achieve the change in coupling strength.

Second, we adopt a similar strategy as that used in simulated annealing. In Simulated annealing, the spins are flipped based on a probability decided by the differences in the energy. Doing the same thing in hardware is a complex process. To simplify the process, we use a "spin fix"; we randomly choose a node and briefly clip it to one of the supply rails. The nodal spin either maintains its current state or swaps to the opposite state. The probability/frequency of spin fixes is determined based on temperature. The temperature follows the same exponential annealing schedule discussed above. In other words, the frequency of spin fixes decays exponentially over time.

\subsection{Theoretical analysis}
We can theoretically define the evolution of above described LDPC decoder using equation~\ref{eqn:rim_node_simplifed}. It shows how the voltage of a capacitor representing each node change over time. $J_{ij}$ represents the effective conductance of the coupling with the parity equations. $B_i$ represents the bias current and  $g_{\!_{ZIV}}(v_{i})$ represents the current due to $ZIV$ diode.

\begin{equation}\label{eqn:rim_node_simplifed}
\begin{split}
    \dv{v_i}{t} = \frac{1}{C}(I_{in} - I_{ZIV}) =  \frac{1}{C} \left[ \sum_{\mathclap{j}} J_{ij} P_{j\backslash i} + B_i - g_{\!_{ZIV}}(v_{i}) \right]
\end{split}
\end{equation}

With this equation, we can provide the same Lyapunov stability analysis as shown in the following paper~\cite{afoakwa.hpca21} to prove our ability for optimum-seeking.


\begin{comment}
\todo{The commented section was not checked in editing -Andrew}

\subsection{Theoretical analysis} \label{ssec:theory}

\todo{Need to be modified}
We present same  Lyapunov stability analysis
of our LDPC decoder to show its ability for optimum-seeking as shown in the following paper~\cite{afoakwa.hpca21}.
Fig.~\ref{fig:brim} shows a simplified node $i$ in LDPC decoder where other nodes are 
coupled into $i$ from the right.
Writing the current equation, we get Eq.~\ref{eqn:rim_node_simplifed}, where $J_{ij}$ is the 
effective conductance of the coupling taking into account the polarity of
the coupling:
\begin{equation}\label{eqn:rim_node_simplifed}
\begin{split}
    \dv{v_i}{t} = \frac{1}{C}(I_{in} - I_{ZIV}) =  \frac{1}{C} \left[ \sum_{\mathclap{j}} J_{ij} P_{j\backslash i} - g_{\!_{ZIV}}(v_{i}) \right]
\end{split}
\end{equation}

LDPC decoder is a continuous time system where the state is summarized by
$v(t)=[v_1(t), v_2(t), ...\,, v_N(t)]^T$. (For brevity, in the following, $v_i(t)$
will be abbreviated as $v_i$.) Recall that in Lyapunov analysis, if a function
$H(v)$ can be found such that $\dv{H(v)}{t} = 0$ at point $v^e$
and $\dv{H(v)}{t} < 0$ in the region around $v^e$, then $v^e$ is the
equilibrium point~\cite{nonlinear_system_analysis}. In our case, this point is the solution to the equation set
$\dv{v_i}{t} = 0;\ i=1..N$.
\donotshow{\footnote{For those unfamiliar with the analysis, here is a roughly
explanation: if the condition $\dv{H(v)}{t} \leq 0$ is satisfied in a region
$v \in W$, that means once the system enters region $W$ at time $t_0$,
function $H(v(t))$ can only decrease or maintain its value (because its time
derivative is non-positive), thus a future state then clearly $H(v)$ can not
increase for a dynamical system can be identified, the system can be shown to
be stable at points where the function reaches minimum.}}
In other words, once the system enters a region, it will inevitably evolve
towards lowering $H(v)$ (because its time derivative is negative) until
it reaches the equilibrium point $v^e$.

To ensure $\dv{H(v)}{t}$ is non-positive, we can construct
it to be in a negative square form. This can be achieved 
by imposing the following construction rule.
\begin{equation}
\label{eqn:rule}
\pdv{H(v)}{v_i}=-\alpha\dv{v_i}{t}; \ \alpha>0
\end{equation} 

Following the chain rule, it is not difficult to see that:
\begin{equation}
\label{eqn:H_partials}
\dv{H(v)}{t} =\sum_{\mathclap{i}}\left(\pdv{H(v)}{v_i}\dv{v_i}{t} \right)
=-\alpha\sum_{\mathclap{i}}\left(\dv{v_i}{t}\right)^2
\end{equation}

One choice of a Lyapunov function satisfying the conditions in Eq.
\ref{eqn:rule} is shown in Eq.~\ref{eqn:Lyap_RIM}, where $G(v_i)$ is obtained
from $g_{\!_{ZIV}}(v_i)$ by integration over $v_i$. 
\begin{equation}
\label{eqn:Lyap_RIM}
H(v)= \frac{\alpha}{C}\Big(-\sum_{\mathclap{i}} \sum_{\mathclap{j}} J_{ij} P_{j\backslash i} v_i + \sum_i G(v_i)\Big)
\end{equation}
It is important to
notice that the ``Z" shape of $g_{\!_{ZIV}}(v)$ will give $P(v)$ a double-well
profile (as shown in Fig.~\ref{fig:brim}-right) with two stable equilibrium points at voltages corresponding to two
non-trivial zero-crossings of the IV curve (\eg $v_i= \pm 1V $) and a saddle
point at $v_i=0V$. Given the double-well profile of $P(v)$, the state of a
stable solution will consist of voltages at (or at least very close to) 
these equilibria (\eg $\pm 1V$).
Thus, the second term of Eq.~\ref{eqn:Lyap_RIM} will be (close to) a constant. 
Consequently, minimizing $H(v)$ is equal to minimizing the first term $-\sum_{i<j}J_{ij}v_iP_{j\backslash i}$, which is the Ising formula.

% \begin{figure}[htp]\centering
%     \includegraphics[width=0.4\textwidth]{double_well.pdf}
%     \caption{\fixme{double well of the -P(v)}}
%     \label{fig:double_well}
% \end{figure}

%Since function $H(v)$ satisfies the conditions in Eq.
%\ref{eqn:H_partials} for all $i's$ representing a sufficient condition
%for $\frac{dH(v)}{dt}=-\sum_{i}\frac{\partial H(v_i)}{\partial
%v_i}\frac{dv_i}{dt}\leq0$, the system is stable in the Lyapunov sense and it
%is guaranteed to converge to a minimum of $H(v)$.

Note that this analysis does not guarantee that the system will converge to a
\emph{global} minimum as it depends on the energy landscape and initial 
conditions. This is similar to other annealers: None 
has strong guarantees for reaching ground state in a typical usage scenario
(as opposed to ideal conditions) or in an efficient manner. For example, it
is shown that simulated annealing can reach ground state in a system with
a finite phase space. However, the time it takes to do so may be longer than
enumerating the space~\cite{varty2017simulated}.
\end{comment}
